Measurement of the Muon Flux at SND@LHC: Results from the 2023-2025 Proton and Heavy-Ion Periods

The SND@LHC experiment investigates neutrinos in the $7.2 < \eta < 8.4$ forward pseudorapidity range. The detector consists of a veto system, a scintillating fiber tracker interleaved with emulsion cloud chambers, and a downstream muon system. Muons originating from collisions at ATLAS (IP1) constitute the primary background for CC neutrino interactions and determine the replacement frequency of the emulsion target. A precise characterization of this flux is therefore essential. In this work, we report the muon flux measured in the central $31 \times 31\text{ cm}^2$ fiducial area of the detector using data from 2023 through 2025. The measured fluxes for $\textbf{proton collisions}$ are: $(1.90 \pm 0.04) \times 10^{-2}\text{ nb/cm}^2$ (2023), $(3.76 \pm 0.09) \times 10^{-2}\text{ nb/cm}^2$ (2024), and $(2.48 \pm 0.05) \times 10^{-2}\text{ nb/cm}^2$ (2025). A 2024 reference proton run at $\sqrt{s} = 5.36\text{ TeV}$ yielded $(4.21 \pm 0.14) \times 10^{-2}\text{ nb/cm}^2$, providing a direct baseline for the heavy-ion energy regime. The measured fluxes for $\textbf{heavy-ion collisions}$ are $(3.11 \pm 0.12) \times 10^4\text{ nb/cm}^2$, $(5.53 \pm 0.22) \times 10^4\text{ nb/cm}^2$, and $(3.24 \pm 0.13) \times 10^4\text{ nb/cm}^2$ in 2023, 2024, and 2025, respectively. Uncertainties are dominated by systematic effects, with the statistical component contributing $\lesssim 0.1\%$ to the total uncertainty. These results are in agreement with Monte Carlo predictions.

==> citations.tex <==
\begin{thebibliography}{99}

\bibitem{bib:sndlhc}
R. Albanese, et al. (SND@LHC Collaboration), ``\textit{Observation of collider muon neutrinos with the SND@LHC experiment}'', Phys. Rev. Lett. \textbf{131}, 031802 (2023), \doi{10.1103/PhysRevLett.131.031802}.

\bibitem{bib:ppMuonFlux}
R. Albanese, et al. (SND@LHC Collaboration), ``\textit{Measurement of the muon flux at the SND@LHC experiment}'', Eur. Phys. J. C \textbf{84}, 90 (2024), \doi{10.1140/epjc/s10052-023-12380-3}.

\bibitem{bib:detector}
G. Acampora, et al., ``\textit{SND@LHC: the scattering and neutrino detector at the LHC}'', JINST \textbf{19}, P05067 (2024), \doi{10.1088/1748-0221/19/05/P05067}.

\bibitem{bib:3rd_veto_plane}
D. Abbaneo, et al. (SND@LHC Collaboration), ``\textit{Installation and performance of the 3rd Veto plane at the SND@LHC detector}'', JINST \textbf{20}, P07011 (2025), \doi{10.1088/1748-0221/20/07/P07011}.

\bibitem{bib:miniDT}
L. Mozzina, ``\textit{Upgrade of the SND@LHC muon detectors with drift tubes}'', M.Sc thesis, Università di Bologna (2025). \url{https://amslaurea.unibo.it/id/eprint/36655/}.

\bibitem{bib:lhc_highlights}
H.~Timko \textit{et al.}, 
``\textit{Highlights from the LHC}'', 
{PoS \textbf{EPS-HEP2025} (2025) 007},
\doi{10.22323/1.485.0007}.

\bibitem{bib:AtlasLumi}
ATLAS Collaboration, ``\textit{Preliminary analysis of the luminosity calibration for the ATLAS 13.6 TeV data recorded in 2023}'', ATL-DAPR-PUB-2024-001, CERN (2024), \url{https://cds.cern.ch/record/2900949}.

\bibitem{bib:FLUKA}
G. Hugo, et al., ``\textit{Status and advances of Monte Carlo codes for particle transport simulation}'', EPJ Nuclear Sci. Technol. \textbf{10}, 20 (2024), \doi{10.1051/epjn/2024023}.

\bibitem{bib:DPMJET}
S. Roesler, R. Engel, and J. Ranft, ``\textit{The Monte Carlo Event Generator DPMJET-III}'', in \textit{Advanced Monte Carlo for Radiation Physics}, 1033--1038, Springer Berlin Heidelberg (2001), \doi{10.1007/978-3-642-18211-2_166}.

\bibitem{bib:Geant4}
S. Agostinelli, et al., ``\textit{Geant4—a simulation toolkit}'', Nucl. Instrum. Meth. A \textbf{506}, 250--303 (2003), \doi{10.1016/S0168-9002(03)01368-8}.



\bibitem{bib:HoughTransform}
P.~V.~C.~Hough, ``\textit{Machine Analysis of Bubble Chamber Pictures}'', Conf. Proc. C \textbf{590914}, 554-558 (1959).

\bibitem{bib:Kalman}
R. E. Kalman, ``\textit{A New Approach to Linear Filtering and Prediction Problems}'', J. Basic Eng. \textbf{82}(1), 35--45 (1960), \doi{10.1115/1.3662552}.

\bibitem{bib:Genfit}
J. Rauch and T. Schlüter, ``\textit{GENFIT — a Generic Track-Fitting Toolkit}'', J. Phys.: Conf. Ser. \textbf{608}, 012042 (2015), \doi{10.1088/1742-6596/608/1/012042}.

\bibitem{bib:CERN_GIS}
CERN, \textit{CERN GIS Portal}, \url{https://gis.cern.ch/} (Accessed: 2025-09-18).

\bibitem{bib:lhc_2022}
D. Jacquet et al., ``\textit{The LHC Run 2022}'', in Proc. IPAC, 551--554 (2023), \doi{10.18429/JACoW-IPAC2023-MOPL020}.

\bibitem{bib:lhc_settings_2023_and_2024}
T. Persson et al., ``\textit{LHC optics commissioning in 2023 and 2024}'', in Proc. IPAC, 67--70 (2024), \doi{10.18429/JACoW-IPAC2024-MOPC12}.

\end{thebibliography}
